Team \'UFAL at CMCL 2022 Shared Task: Figuring out the correct recipe for predicting Eye-Tracking features using Pretrained Language Models

Eye-Tracking data is a very useful source of information to study cognition and especially language comprehension in humans. In this paper, we describe our systems for the CMCL 2022 shared task on predicting eye-tracking information. We describe our experiments with pretrained models like BERT and XLM and the different ways in which we used those representations to predict four eye-tracking features. Along with analysing the effect of using two different kinds of pretrained multilingual language models and different ways of pooling the tokenlevel representations, we also explore how contextual information affects the performance of the systems. Finally, we also explore if factors like augmenting linguistic information affect the predictions. Our submissions achieved an average MAE of 5.72 and ranked 5th in the shared task. The average MAE showed further reduction to 5.25 in post task evaluation.

==> Makefile <==
LATEX=pdflatex
MAINFILE=acl

default: $(MAINFILE).pdf

$(MAINFILE).pdf: custom.bib

%.pdf: %.tex
	$(LATEX) $<
	bibtex $* || ( echo "Bibtex failed" && exit 1 )
	# change the exit 1 to exit 0 in the line above if you want to ignore it
	lim=4; \
	  while [ $$lim -ge 0 ] \
	      && grep 'Rerun to get\|Citation.*undefined' $*.log >/dev/null 2>/dev/null; do \
	    $(LATEX) $< ; \
	    lim=$$(($$lim - 1)) ; \
	  done

.PHONY: ci
ci:
	# make sure git will remember my password
	git config credential.helper store
	# git pull push dance with possibly uncommited local modifications
	if git pull --no-edit; then echo No changes to hide; else git stash; git pull --no-edit; git stash apply; fi; git commit -am "make ci by $(USER)"; git push

clean:
	rm -f $(MAINFILE).log $(MAINFILE).aux $(MAINFILE).bbl $(MAINFILE).blg $(MAINFILE).toc $(MAINFILE).out $(MAINFILE).run.xml $(MAINFILE).bcf

